Learning to Combat Noisy Labels via Classification Margins

A deep neural network trained on noisy labels is known to quickly lose its power to discriminate clean instances from noisy ones. After the early learning phase has ended, the network memorizes the noisy instances, which leads to a significant degradation in its generalization performance. To resolve this issue, we propose MARVEL (MARgins Via Early Learning), a new robust learning method where the memorization of the noisy instances is curbed. We propose a new test statistic that tracks the goodness of "fit" of every instance based on the epoch-history of its classification margins. If its classification margin is small in a sequence of consecutive learning epochs, that instance is declared noisy and the network abandons learning on it. Consequently, the network first flags a possibly noisy instance, and then waits to see if learning on that instance can be improved and if not, the network learns with confidence that this instance can be safely abandoned. We also propose MARVEL+, where arduous instances can be upweighted, enabling the network to focus and improve its learning on them and consequently its generalization. Experimental results on benchmark datasets with synthetic label noise and real-world datasets show that MARVEL outperforms other baselines consistently across different noise levels, with a significantly larger margin under asymmetric noise.

==> tables/binary_asym_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{Boot}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Truck}} \\
Noise     &  &                      (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%)      &  &                       (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%) \\
\midrule
CE         &     &            $93.08\pm1.71$ & $82.38\pm1.84$ & $84.28\pm2.79$ & $78.01\pm1.68$              &     &             $89.05\pm0.82$ & $79.39\pm0.86$ & $78.00\pm1.13$ & $74.35\pm0.78$ \\
%\midrule
GCE       &     &            $96.56\pm0.36$ & $95.96\pm0.26$ & $88.16\pm1.89$ & $87.88\pm1.85$      &     &             $94.06\pm0.37$ & $91.29\pm0.77$ & $78.02\pm0.95$ & $81.72\pm2.15$ \\
SCE        &     &            $96.66\pm0.32$ & $94.98\pm0.77$ & $91.17\pm1.29$ & $89.96\pm1.98$      &     &             $94.18\pm0.31$ & $91.55\pm0.70$ & $82.01\pm2.06$ & $83.01\pm2.17$ \\
NPCL      &     &            $96.78\pm0.32$ & $96.08\pm0.32$ & $94.02\pm1.10$ & $93.56\pm1.43$         &     &             $94.70\pm0.44$ & $92.14\pm0.82$ & $80.17\pm1.83$ & $81.23\pm4.01$ \\
\name     &     &            $\best{96.99}\pm0.18$ & ${\second{96.25}}\pm0.24$ & ${\second{95.22}}\pm0.27$ & ${\second{94.17}}\pm0.57$       &     &           ${\second{95.39}}\pm0.20$ & ${\second{93.39}}\pm0.45$ & ${\second{92.35}}\pm0.57$ & ${\second{88.73}}\pm1.31$ \\
\name+                    &     &            ${\second{96.95}}\pm0.12$ & $\best{96.31}\pm0.27$ & $\best{95.45}\pm0.22$ & $\best{94.96}\pm0.29$       &     &             $\best{95.61}\pm0.23$ & $\best{93.70}\pm0.37$ & $\best{92.94}\pm0.49$ & $\best{89.82}\pm1.12$\\
\midrule
\midrule
Dataset &  & \multicolumn{4}{c}{\textsc{Cat}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Aquatic}} \\
Noise     &  &                      (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%)               &  &                       (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%) \\
\midrule
CE         &     &            $82.14\pm0.80$ & $73.23\pm1.22$ & $72.72\pm1.24$ & $68.06\pm1.31$            &     &             $78.95\pm0.98$ & $71.48\pm1.24$ & $71.30\pm1.51$ & $68.04\pm1.18$ \\
%\midrule
GCE       &     &            $83.71\pm1.32$ & $78.31\pm0.91$ & $72.45\pm1.32$ & $70.25\pm1.33$          &     &             $81.95\pm0.87$ & $78.27\pm1.33$ & $70.73\pm1.22$ & $70.55\pm2.47$ \\
SCE        &     &            $84.80\pm0.89$ & $78.43\pm1.18$ & $72.76\pm1.70$ & $66.54\pm1.41$              &     &             $81.73\pm0.63$ & $77.28\pm1.21$ & $69.41\pm1.13$ & $70.25\pm1.91$ \\
NPCL      &     &            $83.13\pm0.72$ & $76.16\pm1.81$ & $62.04\pm0.91$ & $61.78\pm1.61$        &     &             $81.91\pm0.88$ & $78.47\pm1.35$ & $67.48\pm2.40$ & $68.56\pm2.74$ \\
\name     &     &            ${\second{86.88}}\pm1.45$ & ${\second{81.31}}\pm1.09$ & ${\second{75.52}}\pm1.66$ & ${\second{70.65}}\pm2.34$            &      &             ${\second{82.57}}\pm0.79$ & ${\second{79.15}}\pm1.00$ & ${\second{71.35}}\pm4.69$ & ${\second{71.44}}\pm2.78$ \\
\name+                    &     &             $\best{87.32}\pm0.48$ & $\best{82.28}\pm1.10$ & $\best{77.47}\pm2.25$ & $\best{72.59}\pm1.38$             &     &             $\best{83.62}\pm0.50$ & $\best{80.14}\pm0.92$ & $\best{74.52}\pm1.79$ & $\best{74.04}\pm1.97$ \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Mean $\pm$ standard deviation (over 10 runs) of the test accuracy with asymmetric label noise. 
%Reported are the mean and the standard deviation over 10 runs of the final test accuracy. 
%The highest test accuracy is highlighted in bold.
} \label{table-results-asym}
\begin{adjustbox}{max width=0.9\columnwidth, center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lccccc}
\toprule
\textsc{Method} &  \multicolumn{4}{c}{\cellcolor{gray!50}\textsc{Asymmetric label noise}}\\
%\hline
%\multicolumn{1}{c}{} & \multicolumn{4}{c}{ \cellcolor{gray!50}  {\sc Asymmetric label noise}}\\
\cline{2-5}
& (20\%,0\%) & (30\%,10\%) & (40\%,0\%) & (40\%,10\%)\\
\cline{2-5}

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Boot}}\\
CE & 93.08$\pm$1.71 & 82.38$\pm$1.84 & 84.28$\pm$2.79 & 78.01$\pm$1.68\\
GCE & 96.56$\pm$0.36 & 95.96$\pm$0.26 & 88.16$\pm$1.89 & 87.88$\pm$1.85\\
SCE & 96.66$\pm$0.32 & 94.98$\pm$0.77 & 91.17$\pm$1.29 & 89.96$\pm$1.98\\
NPCL & 96.66$\pm$0.32 & 94.98$\pm$0.77 & 91.17$\pm$1.29 & 89.96$\pm$1.98\\
\name & \textbf{96.99}$\pm$0.18 & {\color{xblue}\textbf{96.25}}$\pm$0.24 & {\color{xblue}\textbf{95.22}}$\pm$0.27 & {\color{xblue}\textbf{94.17}}$\pm$0.57\\
\name+ & {\color{xblue}\textbf{96.95}}$\pm$0.12 & \textbf{96.31}$\pm$0.27 & \textbf{95.45}$\pm$0.22 & \textbf{94.96}$\pm$0.29\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Truck}}\\
CE & 89.05$\pm$0.82 & 79.39$\pm$0.86 & 78.00$\pm$1.13 & 74.35$\pm$0.78\\
GCE & 94.06$\pm$0.37 & 91.29$\pm$0.77 & 78.02$\pm$0.95 & 81.72$\pm$2.15\\
SCE & 94.18$\pm$0.31 & 91.55$\pm$0.70 & 82.01$\pm$2.06 & 83.01$\pm$2.17\\
NPCL & 94.70$\pm$0.44 & 92.14$\pm$0.82 & 80.17$\pm$1.83 & 81.23$\pm$4.01\\
\name & {\color{xblue}\textbf{95.39}}$\pm$0.20 & {\color{xblue}\textbf{93.39}}$\pm$0.45 & {\color{xblue}\textbf{92.35}}$\pm$0.57 &{\color{xblue}\textbf{88.73}}$\pm$1.31\\
\name+ & \textbf{95.61}$\pm$0.23 & \textbf{93.70}$\pm$0.37 & \textbf{92.94}$\pm$0.49 & \textbf{89.82}$\pm$1.12\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Cat}}\\
CE & 82.14$\pm$0.80 & 73.23$\pm$1.22 & 72.72$\pm$1.24 & 68.06$\pm$1.31\\
GCE & 83.71$\pm$1.32 & 78.31$\pm$0.91 & 72.45$\pm$1.32 & 70.25$\pm$1.33\\
SCE & 84.80$\pm$0.89 & 78.43$\pm$1.18 & 72.76$\pm$1.70 & 66.54$\pm$1.41\\
NPCL & 83.13$\pm$0.72 & 76.16$\pm$1.81 & 62.04$\pm$0.91 & 61.78$\pm$1.61\\
\name & {\color{xblue}\textbf{86.88}}$\pm$1.45 & {\color{xblue}\textbf{81.31}}$\pm$1.09 & {\color{xblue}\textbf{75.52}}$\pm$1.66 & {\color{xblue}\textbf{70.65}}$\pm$2.34\\
\name+ &  \textbf{87.32}$\pm$0.48 & \textbf{82.28}$\pm$1.10 & \textbf{77.47}$\pm$2.25 & \textbf{72.59}$\pm$1.38\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Aquatic}}\\
CE & 78.95$\pm$0.98 & 71.48$\pm$1.24 & 71.30$\pm$1.51 & 68.04$\pm$1.18\\
GCE & 81.95$\pm$0.87 & 78.27$\pm$1.33 & 70.73$\pm$1.22 & 70.55$\pm$2.47\\
SCE & 81.73$\pm$0.63 & 77.28$\pm$1.21 & 69.41$\pm$1.13 & 70.25$\pm$1.91\\
NPCL & 81.91$\pm$0.88 & 78.47$\pm$1.35 & 67.48$\pm$2.40 & 68.56$\pm$2.74\\
\name & {\color{xblue}\textbf{82.57}}$\pm$0.79 &{\color{xblue}\textbf{79.15}}$\pm$1.00 &{\color{xblue}\textbf{71.35}}$\pm$4.69 &{\color{xblue}\textbf{71.44}}$\pm$2.78\\
\name+ & \textbf{83.62}$\pm$0.50 & \textbf{80.14}$\pm$0.92 & \textbf{74.52}$\pm$1.79 & \textbf{74.04}$\pm$1.97\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/binary_asym_wait_aaai.tex <==
\begin{tabular}{ccccc}
\toprule
Dataset &   \multicolumn{4}{c}{\textsc{Boot}}                                                                                    \\
Noise     &                        (0.2,0) &                       (0.3,0.1) &                       (0.4,0) &                       (0.4,0.1)      \\
\midrule
\name     &                 6 & 6 & 5 & 6       \\
\name+                    &                 6 & 7 & 5 & 4       \\
\midrule
\midrule
Dataset &      \multicolumn{4}{c}{\textsc{Truck}} \\
Noise     &                                                (0.2,0) &                       (0.3,0.1) &                       (0.4,0) &                       (0.4,0.1)      \\
\midrule
\name     &                                 3 & 4 & 3 & 4 \\
\name+                    &                                   4 & 4 & 3 & 3\\
\midrule
\midrule
Dataset &   \multicolumn{4}{c}{\textsc{Cat}}                                                                                    \\
Noise     &                        (0.2,0) &                       (0.3,0.1) &                       (0.4,0) &                       (0.4,0.1)      \\
\midrule
\name     &                 5 & 4 & 4 & 5            \\
\name+                    &                  5 & 4 & 4 & 5            \\
\midrule
\midrule
Dataset &      \multicolumn{4}{c}{\textsc{Aquatic}} \\
Noise     &                                           (0.2,0) &                       (0.3,0.1) &                       (0.4,0) &                       (0.4,0.1)      \\
\midrule
\name     &                                   4 & 5 & 5 & 6 \\
\name+                    &                                   4 & 5 & 5 & 6 \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Wait period selected via cross validation on different datasets with asymmetric label noise.
%Reported are the mean and the standard deviation over 10 runs of the final test accuracy. 
%The highest test accuracy is highlighted in bold.
} \label{table-hyper-binary-asym}
\begin{adjustbox}{max width=\columnwidth, center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lcccc}
\toprule
\textsc{Method} &  \multicolumn{4}{c}{\cellcolor{gray!50}\textsc{Aymmetric label noise}}\\
%\hline
%\multicolumn{1}{c}{} & \multicolumn{5}{c}{ \cellcolor{gray!50}  {  \sc Symmetric label noise}}\\
\cline{2-5}
& (20\%,0\%) & (30\%,10\%) & (40\%,0\%) & (40\%,10\%)\\
\cline{2-5}

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Boot}}\\
\name & 6 & 6 & 5 & 6\\
\name+ & 6 & 7 & 5 & 4\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Truck}}\\
\name & 3 & 4 & 3 & 4\\
\name+ & 4 & 4 & 3 & 3\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Cat}}\\
\name & 5 & 4 & 4 & 5\\
\name+ & 5 & 4 & 4 & 5\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Aquatic}}\\
\name & 4 & 5 & 5 & 6\\
\name+ & 4 & 5 & 5 & 6\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/binary_asym_wait_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{Boot}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Truck}} \\
Noise     &  &                      (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%)      &  &                       (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%) \\
\midrule
\name     &     &            6 & 6 & 5 & 6       &     &           3 & 4 & 3 & 4 \\
\name+                    &     &            6 & 7 & 5 & 4       &     &             4 & 4 & 3 & 3\\
\midrule
\midrule
Dataset &  & \multicolumn{4}{c}{\textsc{Cat}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Aquatic}} \\
Noise     &  &                      (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%)               &  &                       (20\%,0\%) &                       (30\%,10\%) &                       (40\%,0\%) &                       (40\%,10\%) \\
\midrule
\name     &     &            5 & 4 & 4 & 5            &      &             4 & 5 & 5 & 6 \\
\name+                    &     &             5 & 4 & 4 & 5             &     &             4 & 5 & 5 & 6 \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Wait period selected via cross validation on different datasets with asymmetric label noise.
%Reported are the mean and the standard deviation over 10 runs of the final test accuracy. 
%The highest test accuracy is highlighted in bold.
} \label{table-hyper-binary-asym}
\begin{adjustbox}{max width=\columnwidth, center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lcccc}
\toprule
\textsc{Method} &  \multicolumn{4}{c}{\cellcolor{gray!50}\textsc{Aymmetric label noise}}\\
%\hline
%\multicolumn{1}{c}{} & \multicolumn{5}{c}{ \cellcolor{gray!50}  {  \sc Symmetric label noise}}\\
\cline{2-5}
& (20\%,0\%) & (30\%,10\%) & (40\%,0\%) & (40\%,10\%)\\
\cline{2-5}

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Boot}}\\
\name & 6 & 6 & 5 & 6\\
\name+ & 6 & 7 & 5 & 4\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Truck}}\\
\name & 3 & 4 & 3 & 4\\
\name+ & 4 & 4 & 3 & 3\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Cat}}\\
\name & 5 & 4 & 4 & 5\\
\name+ & 5 & 4 & 4 & 5\\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Aquatic}}\\
\name & 4 & 5 & 5 & 6\\
\name+ & 4 & 5 & 5 & 6\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/binary_sym_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{Boot}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Truck}} \\
Noise     &  &                      10\% &                       20\% &                       30\% &                       40\%      &  &                       10\% &                       20\% &                       30\% &                       40\% \\
\midrule
CE         &     &            $92.04\pm0.76$ & $84.49\pm1.29$ & $74.87\pm2.24$ & $68.28\pm4.33$               &     &             $89.84\pm0.52$ & $81.21\pm1.04$ & $70.33\pm1.27$ & $60.39\pm1.47$ \\
%\midrule
GCE       &     &            $97.10\pm0.18$ & $96.00\pm0.67$ & $\best{96.07}\pm0.31$ & $94.30\pm0.50$      &     &             $94.79\pm0.28$ & $93.31\pm0.44$ & $89.26\pm0.77$ & $75.02\pm1.99$ \\
SCE        &     &            $\best{97.19}\pm0.17$ & $96.41\pm0.47 $& $94.11\pm0.72$ & $89.04\pm2.70$       &     &             $94.80\pm0.31$ & $93.49\pm0.43$ & $89.05\pm1.07$ & $77.56\pm2.40$ \\
NPCL      &     &            $97.10\pm0.24$ & $96.75\pm0.22$ & ${\second{96.04}}\pm0.30$ & $93.13\pm0.61$         &     &             ${\second{95.21}}\pm0.19$ & $93.78\pm0.57$ & ${\second{89.99}}\pm0.76$ & $71.32\pm1.14$ \\
\name     &     &            ${\second{97.13}}\pm0.20$ & ${\second{96.81}}\pm0.21$ & $96.03\pm0.29$ & $\best{94.39}\pm0.44$       &     &           $95.02\pm0.37$ & ${\second{93.87}}\pm0.27$ & $89.93\pm0.51$ & $\best{79.62}\pm1.98$ \\
\name+                    &     &            $97.02\pm0.21$ & $\best{96.85}\pm0.26$ & $95.94\pm0.31$ & ${\second{94.35}}\pm0.48$       &     &             $\best{95.32}\pm0.27$ & $\best{93.94}\pm0.44$ & $\best{90.29}\pm0.51$ & ${\second{79.30}}\pm1.81$\\
\midrule
\midrule
Dataset &  & \multicolumn{4}{c}{\textsc{Cat}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Aquatic}} \\
Noise     &  &                      10\% &                       20\% &                       30\% &                       40\%               &  &                       10\% &                       20\% &                       30\% &                       40\% \\
\midrule
CE         &     &            $81.95\pm0.45$ & $73.43\pm0.79$ & $64.65\pm1.49$ & $56.64\pm1.11$            &     &             $78.56\pm1.04$ & $71.37\pm1.24$ & $63.37\pm1.89$ & $59.28\pm2.03$ \\
%\midrule
GCE       &     &            $86.06\pm0.68$ & ${\second{83.58}}\pm0.68$ & $\best{76.69}\pm1.36$ & $62.99\pm1.81$          &     &             $82.58\pm0.69$ & $80.11\pm1.45$ & $75.63\pm1.77$ & $67.49\pm2.19$ \\
SCE        &     &            $86.66\pm0.51$ & $83.31\pm0.78$ & $74.97\pm1.62$ & $63.21\pm2.06$              &     &             ${\second{83.14}}\pm0.66$ & $80.13\pm1.40$ & $75.88\pm2.18$ & $67.92\pm1.92$ \\
NPCL      &     &            $85.98\pm0.39$ & $82.87\pm0.73$ & $74.93\pm1.90$ & $60.39\pm2.90$          &     &             $82.74\pm0.80$ & $79.93\pm1.05$ & $75.17\pm1.66$ & $65.36\pm2.49$ \\
\name     &     &            ${\second{87.13}}\pm0.40$ &$ 83.34\pm0.81$ & $76.22\pm1.29$ & ${\second{65.62}}\pm1.05$            &      &             $82.98\pm0.90$ & ${\second{80.32}}\pm0.61$ & ${\second{75.95}}\pm1.92$ & ${\second{69.91}}\pm1.89$ \\
\name+                    &     &            $\best{87.69}\pm0.30$ & $\best{83.63}\pm0.87$ & ${\second{76.62}}\pm1.42$ & $\best{66.47}\pm1.96$             &     &             $\best{84.03}\pm0.74$ & $\best{80.86}\pm0.40$ & $\best{76.76}\pm1.67$ & $\best{70.86}\pm1.51$ \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Mean $\pm$ standard deviation (over 10 runs) of the test accuracy with symmetric label noise. 
%Reported are the mean and the standard deviation over 10 runs of the final test accuracy. 
%The highest test accuracy is highlighted in bold.
} \label{table-results}
\begin{adjustbox}{max width=\columnwidth, center}
%\begin{tabular}{@{\extracolsep{-7.0pt}}lccccc}
\begin{tabular}{lccccc}
\toprule
\textsc{Method} &  \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Symmetric label noise}}\\
%\hline
%\multicolumn{1}{c}{} & \multicolumn{5}{c}{ \cellcolor{gray!50}  {  \sc Symmetric label noise}}\\
\cline{2-6}
& 0\% & 10\% & 20\% & 30\% & 40\%\\
\cline{2-6}

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{gray!50}\textsc{Boot}}\\
%\cdashline{3-8}

CE & \textbf{97.86}$\pm$0.24 & 92.04$\pm$0.76 & 84.49$\pm$1.29 & 74.87$\pm$2.24 & 68.28$\pm$4.33\\
GCE & {\color{xblue}\textbf{97.72}}$\pm$0.21 & 97.10$\pm$0.18 & 96.00$\pm$0.67 & \textbf{96.07}$\pm$0.31 & 94.30$\pm$0.50\\
SCE & 97.61$\pm$0.22 & \textbf{97.19}$\pm$0.17 & 96.41$\pm$0.47 & 94.11$\pm$0.72 & 89.04$\pm$2.70\\
NPCL & 97.50$\pm$0.12 & 97.10$\pm$0.24 & 96.75$\pm$0.22 & {\color{xblue}\textbf{96.04}}$\pm$0.30 & 93.13$\pm$0.61\\
\name & 97.45$\pm$0.09 & {\color{xblue}\textbf{97.13}}$\pm$0.20 & {\color{xblue}\textbf{96.81}}$\pm$0.21 & 96.03$\pm$0.29 & \textbf{94.39}$\pm$0.44\\
\name+ & 97.21$\pm$0.18 & 97.02$\pm$0.21 & \textbf{96.85}$\pm$0.26 & 95.94$\pm$0.31 & {\color{xblue}\textbf{94.35}}$\pm$0.48\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{gray!50}\textsc{Truck}}\\
CE & \textbf{96.51}$\pm$0.33 & 89.84$\pm$0.52 & 81.21$\pm$1.04 & 70.33$\pm$1.27 & 60.39$\pm$1.47\\
GCE & {\color{xblue}\textbf{96.45}}$\pm$0.34 & 94.79$\pm$0.28 & 93.31$\pm$0.44 & 89.26$\pm$0.77 & 75.02$\pm$1.99\\
SCE & 96.36$\pm$0.22 & 94.80$\pm$0.31 & 93.49$\pm$0.43 & 89.05$\pm$1.07 & 77.56$\pm$2.40\\
NPCL & 96.44$\pm$0.27 & {\color{xblue}\textbf{95.21}}$\pm$0.19 & 93.78$\pm$0.57 & {\color{xblue}\textbf{89.99}}$\pm$0.76 & 71.32$\pm$1.14\\
\name & 96.30$\pm$0.30 & 95.02$\pm$0.37 & {\color{xblue}\textbf{93.87}}$\pm$0.27 & 89.93$\pm$0.51 & \textbf{79.62}$\pm$1.98\\
\name+ & 96.27$\pm$0.14 & \textbf{95.32}$\pm$0.27 & \textbf{93.94}$\pm$0.44 & \textbf{90.29}$\pm$0.51 & {\color{xblue}\textbf{79.30}}$\pm$1.81\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{gray!50}\textsc{Cat}}\\
CE & 89.97$\pm$0.39 & 81.95$\pm$0.45 & 73.43$\pm$0.79 & 64.65$\pm$1.49 & 56.64$\pm$1.11\\
GCE & 90.06$\pm$0.34 & 86.06$\pm$0.68 &{\color{xblue}\textbf{83.58}}$\pm$0.68 & \textbf{76.69}$\pm$1.36 & 62.99$\pm$1.81\\
SCE & \textbf{90.47}$\pm$0.50 & 86.66$\pm$0.51 & 83.31$\pm$0.78 & 74.97$\pm$1.62 & 63.21$\pm$2.06\\
NPCL & 87.98$\pm$0.61 & 85.98$\pm$0.39 & 82.87$\pm$0.73 & 74.93$\pm$1.90 & 60.39$\pm$2.90 \\
\name & 89.61$\pm$0.35 & {\color{xblue}\textbf{87.13}}$\pm$0.40 & 83.34$\pm$0.81 & 76.22$\pm$1.29 & {\color{xblue}\textbf{65.62}}$\pm$1.05\\
\name+ & {\color{xblue}\textbf{90.16}}$\pm$0.41 & \textbf{87.69}$\pm$0.30 & \textbf{83.63}$\pm$0.87 & {\color{xblue}\textbf{76.62}}$\pm$1.42 & \textbf{66.47}$\pm$1.96\\
  
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{gray!50}\textsc{Aquatic}}\\
CE & 85.16$\pm$0.68 & 78.56$\pm$1.04 & 71.37$\pm$1.24 & 63.37$\pm$1.89 & 59.28$\pm$2.03\\
GCE & 85.19$\pm$0.87 & 82.58$\pm$0.69 & 80.11$\pm$1.45 & 75.63$\pm$1.77 & 67.49$\pm$2.19\\
SCE & 84.35$\pm$0.44 & {\color{xblue}\textbf{83.14}}$\pm$0.66 & 80.13$\pm$1.40 & 75.88$\pm$2.18 & 67.92$\pm$1.92\\
NPCL & 84.79$\pm$0.80 & 82.74$\pm$0.80 & 79.93$\pm$1.05 & 75.17$\pm$1.66 & 65.36$\pm$2.49\\
\name & \textbf{85.99}$\pm$0.45 & 82.98$\pm$0.90 & {\color{xblue}\textbf{80.32}}$\pm$0.61 & {\color{xblue}\textbf{75.95}}$\pm$1.92 & {\color{xblue}\textbf{69.91}}$\pm$1.89\\
\name+ & {\color{xblue}\textbf{85.83}}$\pm$0.62 & \textbf{84.03}$\pm$0.74 & \textbf{80.86}$\pm$0.40 & \textbf{76.76}$\pm$1.67&\textbf{70.86}$\pm$1.51\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/binary_sym_wait_aaai.tex <==
\begin{tabular}{ccccc}
\toprule
Dataset &   \multicolumn{4}{c}{\textsc{Boot}}                                                                                    \\
Noise     &                        10\% &                       20\% &                       30\% &                       40\%      \\
\midrule
\name     &                6 & 6 & 5 & 6         \\
\name+                    &                 6 & 6 & 5 & 6       \\
\midrule
\midrule
Dataset &      \multicolumn{4}{c}{\textsc{Truck}} \\
Noise     &                                         10\% &                       20\% &                       30\% &                       40\% \\
\midrule
\name     &                                5 & 3 & 4 & 4 \\
\name+                    &                                   5 & 3 & 4 & 4\\
\midrule
\midrule
Dataset &   \multicolumn{4}{c}{\textsc{Cat}}                                                                                     \\
Noise     &                        10\% &                       20\% &                       30\% &                       40\%               \\
\midrule
\name     &                 4 & 4 & 5 & 5            \\
\name+                    &                 4 & 5 & 5 & 5              \\
\midrule
\midrule
Dataset &      \multicolumn{4}{c}{\textsc{Aquatic}} \\
Noise     &                                                 10\% &                       20\% &                       30\% &                       40\% \\
\midrule
\name     &                                   4 & 4 & 4 & 5 \\
\name+                    &                                  7 & 4 & 4 & 6 \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Wait period selected via cross validation on different datasets with symmetric label noise.
%Reported are the mean and the standard deviation over 10 runs of the final test accuracy. 
%The highest test accuracy is highlighted in bold.
} \label{table-hyper-binary}
\begin{adjustbox}{max width=\columnwidth, center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lccccc}
\toprule
\textsc{Method} &  \multicolumn{5}{c}{\cellcolor{gray!50}\textsc{Symmetric label noise}}\\
%\hline
%\multicolumn{1}{c}{} & \multicolumn{5}{c}{ \cellcolor{gray!50}  {  \sc Symmetric label noise}}\\
\cline{2-6}
& 0\% & 10\% & 20\% & 30\% & 40\%\\
\cline{2-6}

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Boot}}\\
\name & 6 & 6 & 6 & 5 & 6\\
\name+ & 6 & 6 & 6 & 5 & 6\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Truck}}\\
\name & 5 & 5 & 3 & 4 & 4\\
\name+ & 7 & 5 & 3 & 4 & 4\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Cat}}\\
\name & 6 & 4 & 4 & 5 & 5\\
\name+ & 7 & 4 & 5 & 5 & 5\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Aquatic}}\\
\name & 5 & 4 & 4 & 4 & 5\\
\name+ & 5 & 7 & 4 & 4 & 6\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/binary_sym_wait_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{Boot}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Truck}} \\
Noise     &  &                      10\% &                       20\% &                       30\% &                       40\%      &  &                       10\% &                       20\% &                       30\% &                       40\% \\
\midrule
\name     &     &            6 & 6 & 5 & 6        &     &           5 & 3 & 4 & 4 \\
\name+                    &     &            6 & 6 & 5 & 6       &     &             5 & 3 & 4 & 4\\
\midrule
\midrule
Dataset &  & \multicolumn{4}{c}{\textsc{Cat}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Aquatic}} \\
Noise     &  &                      10\% &                       20\% &                       30\% &                       40\%               &  &                       10\% &                       20\% &                       30\% &                       40\% \\
\midrule
\name     &     &            4 & 4 & 5 & 5            &      &             4 & 4 & 4 & 5 \\
\name+                    &     &            4 & 5 & 5 & 5             &     &             7 & 4 & 4 & 6 \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Wait period selected via cross validation on different datasets with symmetric label noise.
%Reported are the mean and the standard deviation over 10 runs of the final test accuracy. 
%The highest test accuracy is highlighted in bold.
} \label{table-hyper-binary}
\begin{adjustbox}{max width=\columnwidth, center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lccccc}
\toprule
\textsc{Method} &  \multicolumn{5}{c}{\cellcolor{gray!50}\textsc{Symmetric label noise}}\\
%\hline
%\multicolumn{1}{c}{} & \multicolumn{5}{c}{ \cellcolor{gray!50}  {  \sc Symmetric label noise}}\\
\cline{2-6}
& 0\% & 10\% & 20\% & 30\% & 40\%\\
\cline{2-6}

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Boot}}\\
\name & 6 & 6 & 6 & 5 & 6\\
\name+ & 6 & 6 & 6 & 5 & 6\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Truck}}\\
\name & 5 & 5 & 3 & 4 & 4\\
\name+ & 7 & 5 & 3 & 4 & 4\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Cat}}\\
\name & 6 & 4 & 4 & 5 & 5\\
\name+ & 7 & 4 & 5 & 5 & 5\\

\multicolumn{1}{c}{} & \multicolumn{5}{c}{\cellcolor{xblue!50}\textsc{Aquatic}}\\
\name & 5 & 4 & 4 & 4 & 5\\
\name+ & 5 & 7 & 4 & 4 & 6\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/cifar10_resnet34_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Type &  & \multicolumn{4}{c}{\textsc{Symmetric}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Class-Dependent}} \\
Noise     &  &                      20\% &                       40\% &                       60\% &                       80\%      &  &                       10\% &                       20\% &                       30\% &                       40\% \\
\midrule
CE         &     &            $81.42\pm0.29$ & $61.24\pm1.41$ & $37.30\pm1.89$ & $29.69\pm2.51$               &     &             $90.68\pm0.18$ & $86.24\pm0.43$ & $81.47\pm0.46$ & $76.12\pm0.65$ \\
%\midrule
SCE        &     &            $90.24\pm0.16$ & $86.86\pm0.23$ & $80.89\pm0.13$ & $\best{43.89}\pm0.91$       &     &             $91.48\pm0.11$ & $90.12\pm0.17$ & $88.02\pm0.12$ & $84.29\pm0.58$ \\
\name     &     &            $\best{92.51}\pm0.34$ & ${\second{89.20}}\pm0.26$ & ${\second{82.16}}\pm2.15$ & ${\second{42.09}}\pm2.05$       &     &           $\best{93.70}\pm0.25$ & ${\second{92.80}}\pm0.25$ & ${\second{91.78}}\pm0.29$ & ${\second{90.60}}\pm0.32$ \\
\name+                    &     &            ${\second{92.20}}\pm0.20$ & $\best{89.45}\pm0.33$ & $\best{82.23}\pm1.22$ & $37.88\pm2.63$       &     &            ${\second{93.59}}\pm0.19$ & $\best{93.09}\pm0.18$ & $\best{91.98}\pm0.37$ & $\best{90.76}\pm0.50$ \\
\midrule
Oracle       &     &            $92.56\pm0.15$ & $91.37\pm0.37$ & $88.99\pm0.36$ & $83.23\pm1.20$      &     &             $93.48\pm0.12$ & $93.25\pm0.10$ & $92.76\pm0.39$ & $92.38\pm0.08$ \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Mean $\pm$ standard deviation (over 5 runs) of the test accuracy on CIFAR-10, at the epoch with lowest validation error, except for \CE, whose final test accuracy is reported. 
%The highest test accuracy \emph{apart from} the oracle method is highlighted in bold. 
%The oracle method trains on the clean data only.
} \label{table-multi}
\begin{adjustbox}{max width=\columnwidth, center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lcccc}
\toprule
\textsc{Method} &  \multicolumn{4}{c}{\textsc{Test accuracy}}\\
%\hline
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Symmetric label noise}}\\
\cline{2-5}
& 20\% & 40\% & 60\% & 80\%\\
CE & 81.42$\pm$0.29 & 61.24$\pm$1.41 & 37.30$\pm$1.89 & 29.69$\pm$2.51\\
SCE & 90.24$\pm$0.16 & 86.86$\pm$0.23 & 80.89$\pm$0.13 & {\color{xblue}\textbf{43.89}}$\pm$0.91\\
ELR & 90.91$\pm$0.20 & 88.22$\pm$0.20 & \textbf{83.33}$\pm$0.58 & \textbf{46.62}$\pm$1.79\\
\name & \textbf{92.51}$\pm$0.34 & {\color{xblue}\textbf{89.20}}$\pm$0.26 & 82.16$\pm$2.15 & 42.09$\pm$2.05\\
\name+ & {\color{xblue}\textbf{92.20}}$\pm$0.20 & \textbf{89.45}$\pm$0.33 & {\color{xblue}\textbf{82.23}}$\pm$1.22 & 37.88$\pm$2.63\\
\hdashline[0.9pt/5pt]
Oracle & 92.56$\pm$0.15 & 91.37$\pm$0.37 & 88.99$\pm$0.36 & 83.23$\pm$1.20\\

\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Asymmetric label noise}}\\
\cline{2-5}
&10\% & 20\% & 30\% & 40\% \\
CE & 90.68$\pm$0.18 & 86.24$\pm$0.43 & 81.47$\pm$0.46 & 76.12$\pm$0.65\\
SCE & 91.48$\pm$0.11 & 90.12$\pm$0.17 & 88.02$\pm$0.12 & 84.29$\pm$0.58\\
ELR & 92.58$\pm$0.18 & 91.55$\pm$0.33 & 90.23$\pm$0.30 & 87.70$\pm$0.33\\
\name & \textbf{93.70}$\pm$0.25 & {\color{xblue}\textbf{92.80}}$\pm$0.25 & {\color{xblue}\textbf{91.78}}$\pm$0.29 & {\color{xblue}\textbf{90.60}}$\pm$0.32\\
\name+ & {\color{xblue}\textbf{93.59}}$\pm$0.19 & \textbf{93.09}$\pm$0.18 & \textbf{91.98}$\pm$0.37 & \textbf{90.76}$\pm$0.50\\
\hdashline[0.9pt/5pt]
Oracle & 93.48$\pm$0.12 & 93.25$\pm$0.10 & 92.76$\pm$0.39 & 92.38$\pm$0.08\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/cifar10_resnet34_wait_aaai.tex <==
\begin{tabular}{ccccc}
\toprule
Type &   \multicolumn{4}{c}{\textsc{Symmetric}}                                                                                       \\
Noise     &                        20\% &                       40\% &                       60\% &                       80\%       \\
\midrule
\name     &                 5 & 4 & 5 & 20        \\
\name+                    &                 6 & 5 & 6 & 25        \\
\midrule
\midrule
Type &    \multicolumn{4}{c}{\textsc{Class-Dependent}} \\
Noise     &                                                10\% &                       20\% &                       30\% &                       40\% \\
\midrule
\name     &                                 6 & 6 & 5 & 4 \\
\name+                    &                                  7 & 6 & 5 & 4 \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Wait periods selected on CIFAR-10 with symmetric and asymmetric label noise.
} \label{table-hyper-multi}
\begin{adjustbox}{max width=\columnwidth,center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lcccc}
\toprule
\textsc{Method} &  \multicolumn{4}{c}{\textsc{Wait period}}\\
%\hline
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Symmetric label noise}}\\
\cline{2-5}
& 20\% & 40\% & 60\% & 80\%\\
\name & 5 & 4 & 5 & 20\\
\name+ & 6 & 5 & 6 & 25\\
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Asymmetric label noise}}\\
\cline{2-5}
& 10\% & 20\% & 30\% & 40\%\\
\name & 6 & 6 & 5 & 4\\
\name+ & 7 & 6 & 5 & 4\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/cifar10_resnet34_wait_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Type &  & \multicolumn{4}{c}{\textsc{Symmetric}}                                                                                    &  & \multicolumn{4}{c}{\textsc{Class-Dependent}} \\
Noise     &  &                      20\% &                       40\% &                       60\% &                       80\%      &  &                       10\% &                       20\% &                       30\% &                       40\% \\
\midrule
\name     &     &            5 & 4 & 5 & 20       &     &           6 & 6 & 5 & 4 \\
\name+                    &     &            6 & 5 & 6 & 25       &     &            7 & 6 & 5 & 4 \\
\bottomrule
\end{tabular}

\iffalse
\begin{table}[ht]
\caption{Wait periods selected on CIFAR-10 with symmetric and asymmetric label noise.
} \label{table-hyper-multi}
\begin{adjustbox}{max width=\columnwidth,center}
\begin{tabular}{@{\extracolsep{-7.0pt}}lcccc}
\toprule
\textsc{Method} &  \multicolumn{4}{c}{\textsc{Wait period}}\\
%\hline
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Symmetric label noise}}\\
\cline{2-5}
& 20\% & 40\% & 60\% & 80\%\\
\name & 5 & 4 & 5 & 20\\
\name+ & 6 & 5 & 6 & 25\\
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\cellcolor{xblue!50}\textsc{Asymmetric label noise}}\\
\cline{2-5}
& 10\% & 20\% & 30\% & 40\%\\
\name & 6 & 6 & 5 & 4\\
\name+ & 7 & 6 & 5 & 4\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
\fi


==> tables/cifar_asym_aaai.tex <==
\begin{tabular}{ccccc}
\toprule
 &  \multicolumn{2}{c}{\textsc{CIFAR-10}} &      \multicolumn{2}{c}{\textsc{CIFAR-100}} \\
 &                       20\% &                       40\% &                       20\% &                       40\% \\
\midrule
CE                                   &                 $81.9\pm0.9$ & $62.5\pm1.8$ &                              $60.5\pm0.2$ & $44.8\pm0.8$             \\
SC                                   &                 $88.8\pm0.2$ & $76.7\pm1.7$ &                              $56.5\pm0.5$ & $43.5\pm0.5$            \\
%Random                                     &             $16.1 \pm 0.2$ &             $34.8 \pm 1.3$ &             $42.3 \pm 0.2$ &             $57.1 \pm 0.2$ \\
BT         &            $76.2 \pm 0.2$ &             $55.0 \pm 0.6$ &             $53.4 \pm 0.3$ &             $38.7 \pm 0.3$ \\
D2                      &             $88.6 \pm 0.2$ &             $76.4 \pm 1.5$ &            $43.6 \pm 0.7$ &             $16.9 \pm 1.2$ \\
L         &             $86.7 \pm 0.8$ &  $84.0 \pm 2.1$ &                   Diverged &                   Diverged \\
DP          &             $82.1 \pm 0.2$ &             $55.5 \pm 0.7$ &             $56.2 \pm 0.5$ &             $39.0 \pm 0.4$ \\
D &             $77.9 \pm 0.1$ &             $59.4 \pm 0.6$ &             $53.2 \pm 0.0$ &             $37.9 \pm 0.0$ \\
IN                  &             $88.3 \pm 0.1$ &             $79.8 \pm 0.4$ &             $56.8 \pm 0.1$ &  $44.4 \pm 0.7$ \\
A                                     &     $89.7 \pm 0.1$ &             $58.7 \pm 0.2$ &       $59.7 \pm 0.2$ &             $40.2 \pm 0.1$ \\
M                                &                 $\best{91.5}\pm0.2$ & $\best{89.4}\pm0.3$ &                             $\best{67.8}\pm0.2$ & $\best{60.6}\pm0.3$             \\
+                               &                 ${\second{91.4}}\pm0.2$ & ${\second{88.7}}\pm0.2$ &                             ${\second{67.5}}\pm0.3$ & ${\second{59.5}}\pm0.4$            \\
\midrule
O                                 &                 $91.5\pm0.2$ & $90.1\pm0.2$ &                              $67.5\pm0.4$ & $65.1\pm0.4$             \\
\bottomrule
\end{tabular}


==> tables/cifar_asym_full.tex <==
\begin{tabular}{ccccccc}
\toprule
Dataset & & \multicolumn{2}{c}{\textsc{CIFAR-10}} &     & \multicolumn{2}{c}{\textsc{CIFAR-100}} \\
Noise &  &                     20\% &                       40\% &      &                 20\% &                       40\% \\
\midrule
CE                                   &     &            $81.92\pm0.89$ & $62.54\pm1.81$ &                 &             $60.51\pm0.23$ & $44.76\pm0.78$             \\
SCE                                   &     &            $88.81\pm0.22$ & $76.68\pm1.67$ &                 &             $56.47\pm0.50$ & $43.45\pm0.47$            \\
%Random                                     &             $16.1 \pm 0.2$ &             $34.8 \pm 1.3$ &             $42.3 \pm 0.2$ &             $57.1 \pm 0.2$ \\
Bootstrap         &   &         $76.2 \pm 0.2$ &             $55.0 \pm 0.6$ &      &       $53.4 \pm 0.3$ &             $38.7 \pm 0.3$ \\
D2L                      &    &         $88.6 \pm 0.2$ &             $76.4 \pm 1.5$ &       &     $43.6 \pm 0.7$ &             $16.9 \pm 1.2$ \\
L\textsubscript{DMI}         &   &          $86.7 \pm 0.8$ &  $84.0 \pm 2.1$ &       &            Diverged &                   Diverged \\
Data Parameters          &   &          $82.1 \pm 0.2$ &             $55.5 \pm 0.7$ &     &        $56.2 \pm 0.5$ &             $39.0 \pm 0.4$ \\
DY-Bootstrap &   &          $77.9 \pm 0.1$ &             $59.4 \pm 0.6$ &    &         $53.2 \pm 0.0$ &             $37.9 \pm 0.0$ \\
INCV                  &    &         $88.3 \pm 0.1$ &             $79.8 \pm 0.4$ &     &        $56.8 \pm 0.1$ &  $44.4 \pm 0.7$ \\
AUM                                     &   &  $89.7 \pm 0.1$ &             $58.7 \pm 0.2$ &  &     $59.7 \pm 0.2$ &             $40.2 \pm 0.1$ \\
\name                                &     &            $\best{91.48}\pm0.18$ & $\best{89.39}\pm0.31$ &                 &             $\best{67.81}\pm0.16$ & $\best{60.57}\pm0.27$             \\
\name+                               &     &            ${\second{91.40}}\pm0.18$ & ${\second{88.66}}\pm0.19$ &                 &            ${\second{67.45}}\pm0.34$ & ${\second{59.50}}\pm0.38$            \\
\midrule
Oracle                                  &     &            $91.49\pm0.20$ & $90.05\pm0.16$ &                 &             $67.50\pm0.43$ & $65.08\pm0.43$             \\
\bottomrule
\end{tabular}


==> tables/cifar_asym_wait_full.tex <==
\begin{tabular}{ccccccc}
\toprule
Dataset & & \multicolumn{2}{c}{\textsc{CIFAR-10}} &     & \multicolumn{2}{c}{\textsc{CIFAR-100}} \\
Noise &  &                     20\% &                       40\% &      &                 20\% &                       40\% \\
\midrule
\name                                &     &            8 &             6 &                 &             16 &             7             \\
\name+                               &     &            10 &             6 &                 &             15 &             6             \\
\bottomrule
\end{tabular}


==> tables/cifar_sym_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{CIFAR-10}} &  & \multicolumn{4}{c}{\textsc{CIFAR-100}} \\
Noise &  &                      20\% &                       40\% &                       60\% &                       80\% &  &                       20\% &                       40\% &                       60\% &                       80\% \\
\midrule
CE                                   &     &            $82.31\pm0.65$ & $72.15\pm0.70$ & $51.33\pm0.90$ & $29.03\pm2.76$ &     &             $58.83\pm0.35$ & $50.49\pm0.32$ & $38.55\pm0.94$ & $17.21\pm1.10$ \\
SCE                                   &     &           $89.46\pm0.09$ & $86.23\pm0.11$ & $78.48\pm0.25$ & $42.80\pm4.57$ &     &             $55.57\pm0.47$ & $45.44\pm0.71$ & $31.76\pm1.12$ & $14.20\pm2.37$ \\
%Random                                     &     &            $16.5 \pm 0.3$ &             $22.8 \pm 0.8$ &             $35.8 \pm 1.4$ &             $55.6 \pm 2.8$ &     &             $43.0 \pm 0.1$ &             $51.2 \pm 0.2$ &             $63.5 \pm 0.5$ &             $83.7 \pm 0.9$ \\
Bootstrap         &     &            $77.6 \pm 0.2$ &             $62.6 \pm 0.4$ &             $48.0 \pm 0.2$ &             $31.2 \pm 0.5$ &     &             $51.4 \pm 0.2$ &             $41.1 \pm 0.2$ &             $29.7 \pm 0.2$ &             $10.2 \pm 0.8$ \\
MentorNet       &     &            $86.7 \pm 0.1$ &             $81.9 \pm 0.2$ &                       --- &             $34.0 \pm 2.5$ &     &             $64.2 \pm 0.3$ &             $57.5 \pm 0.2$ &                       --- &             $24.3 \pm 0.7$ \\
Co-Teaching      &     &            $88.8 \pm 0.1$ &             $86.5 \pm 0.1$ &             $80.7 \pm 0.1$ &             $19.3 \pm 0.6$ &     &             $64.1 \pm 0.1$ &             $60.2 \pm 0.2$ &             $48.0 \pm 0.3$ &             $10.9 \pm 0.7$ \\
D2L                      &     &            $87.7 \pm 0.2$ &             $84.4 \pm 0.3$ &             $72.7 \pm 0.6$ &                   Diverged &     &             $54.0 \pm 1.0$ &             $29.7 \pm 1.8$ &                   Diverged &                   Diverged \\
L\textsubscript{DMI}         &     &            $85.9 \pm 0.1$ &             $79.6 \pm 0.8$ &             $65.1 \pm 1.2$ &             $32.8 \pm 1.4$ &     &                   Diverged &                   Diverged &                   Diverged &                   Diverged \\
Data Parameters          &     &            $82.1 \pm 0.2$ &             $70.8 \pm 0.9$ &             $49.3 \pm 0.7$ &             $18.9 \pm 0.3$ &     &             $56.3 \pm 1.4$ &             $46.1 \pm 0.4$ &             $32.8 \pm 2.3$ &             $11.9 \pm 1.2$ \\
DY-Bootstrap  &     &            $79.4 \pm 0.1$ &             $68.8 \pm 1.4$ &             $56.4 \pm 1.7$ &                   Diverged &     &             $53.0 \pm 0.4$ &             $43.0 \pm 0.3$ &             $36.6 \pm 0.5$ &             $12.8 \pm 0.5$ \\
INCV                  &     &            $89.5 \pm 0.1$ &             $86.8 \pm 0.1$ &             $81.1 \pm 0.3$ &  ${\second{53.3}} \pm 1.9$ &     &             $58.6 \pm 0.5$ &             $55.4 \pm 0.2$ &             $43.7 \pm 0.3$ &             $23.7 \pm 0.6$ \\
AUM                                        &     &  $90.2 \pm 0.0$ &  $87.5 \pm 0.1$ &  $82.1 \pm 0.0$ &  $\best{54.4} \pm 1.6$ &     &  $65.5 \pm 0.2$ &  $61.3 \pm 0.1$ &  $53.0 \pm 0.5$ &  $\best{31.7} \pm 0.7$ \\
\name                                &     &            $\best{91.13}\pm0.20$ & ${\second{88.40}}\pm0.17$ & $\best{83.11}\pm0.14$ & $52.11\pm4.24$ &     &             ${\second{67.50}}\pm0.21$ & $\best{63.84}\pm0.24$ & ${\second{56.80}}\pm0.34$ & ${\second{31.28}}\pm2.20$ \\
\name+                               &     &            ${\second{90.95}}\pm0.19$ & $\best{88.42}\pm0.21$ & ${\second{82.98}}\pm0.24$ & $48.36\pm3.90$ &     &             $\best{67.71}\pm0.14$ & ${\second{63.55}}\pm0.32$ & $\best{56.85}\pm0.71$ & $30.92\pm1.76$ \\
\midrule
Oracle                                  &     &            $91.28\pm0.25$ & $90.00\pm0.21$ & $87.98\pm0.35$ & $83.51\pm1.28$ &     &             $67.64\pm0.23$ & $64.81\pm0.50$ & $60.76\pm0.60$ & $51.27\pm0.41$ \\
\bottomrule
\end{tabular}


==> tables/cifar_sym_wait_aaai.tex <==
\begin{tabular}{ccccc}
\toprule
Dataset &   \multicolumn{4}{c}{\textsc{CIFAR-10}}  \\
Noise &                        20\% &                       40\% &                       60\% &                       80\%  \\
\midrule
\name                                &                 10 &             8 &             8 &             22  \\
\name+                               &                 9 &             7 &             7 &             26  \\
\midrule
\midrule
Dataset &      \multicolumn{4}{c}{\textsc{CIFAR-100}} \\
Noise &                                                 20\% &                       40\% &                       60\% &                       80\% \\
\midrule
\name                                      &            19 &             19 &             16 &             19 \\
\name+                                   &              19 &             18 &             17 &             18 \\
\bottomrule
\end{tabular}


==> tables/cifar_sym_wait_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{CIFAR-10}} &  & \multicolumn{4}{c}{\textsc{CIFAR-100}} \\
Noise &  &                      20\% &                       40\% &                       60\% &                       80\% &  &                       20\% &                       40\% &                       60\% &                       80\% \\
\midrule
\name                                &     &            10 &             8 &             8 &             22 &     &             19 &             19 &             16 &             19 \\
\name+                               &     &            9 &             7 &             7 &             26 &     &             19 &             18 &             17 &             18 \\
\bottomrule
\end{tabular}


==> tables/cifar_tune_wait_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{CIFAR-10 40\% Symmetric}}                                                                                    &  & \multicolumn{4}{c}{\textsc{CIFAR-10 40\% Asymmetric}} \\
Wait     &  &                      6 &                       8 &                       10 &                       12      &  &                       4 &                       6 &                       8 &                       10 \\
\midrule
\name     &     &            $88.37\pm0.20$ & $\select{88.40}\pm0.17$ & $88.21\pm0.21$ & $88.01\pm0.13$        &     &           $88.88\pm0.15$ & $\select{89.39}\pm0.31$ & $89.28\pm0.15$ & $88.68\pm0.13$ \\
\midrule
\midrule
Dataset &  & \multicolumn{4}{c}{\textsc{CIFAR-100 60\% Symmetric}}                                                                                    &  & \multicolumn{4}{c}{\textsc{CIFAR-100 20\% Asymmetric}} \\
Wait     &  &                      10 &                       13 &                       16 &                       19               &  &                       10 &                       13 &                       16 &                       19 \\
\midrule
\name     &     &            $55.80\pm0.32$ & $56.62\pm0.50$ & $\select{56.80}\pm0.34$ & $56.73\pm0.34$            &      &             $67.62\pm0.14$ & $67.71\pm0.23$ & $\select{67.81}\pm0.16$ & $67.55\pm0.17$ \\
\bottomrule
\end{tabular}


==> tables/cifar_tune_warmup_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \multicolumn{4}{c}{\textsc{CIFAR-10 40\% Symmetric}}                                                                                    &  & \multicolumn{4}{c}{\textsc{CIFAR-10 40\% Asymmetric}} \\
Warm-up     &  &                      20 &                       30 &                       40 &                       50      &  &                       20 &                       30 &                       40 &                       50 \\
\midrule
\name     &     &            $88.35\pm0.21$ & $\select{88.40}\pm0.17$ & $88.56\pm0.19$ & $88.26\pm0.31$        &     &           $88.90\pm0.23$ & $\select{89.39}\pm0.31$ & $89.57\pm0.07$ & $89.69\pm0.06$ \\
\midrule
\midrule
Dataset &  & \multicolumn{4}{c}{\textsc{CIFAR-100 60\% Symmetric}}                                                                                    &  & \multicolumn{4}{c}{\textsc{CIFAR-100 20\% Asymmetric}} \\
Warm-up     &  &                      20 &                       30 &                       40 &                       50      &  &                       20 &                       30 &                       40 &                       50 \\
\midrule
\name     &     &            $55.28\pm0.45$ & $56.61\pm0.23$ & $\select{56.80}\pm0.34$ & $56.73\pm0.36$            &      &             $67.36\pm0.15$ & $67.59\pm0.24$ & $\select{67.81}\pm0.16$ & $67.36\pm0.33$ \\
\bottomrule
\end{tabular}

==> tables/real_world_full.tex <==
\begin{tabular}{ccccccccccc}
\toprule
Dataset &  & \textsc{WebVision50} &  & \textsc{Clothing100K} \\
\midrule
CE                                   &     &            $73.10\pm0.37$ & & $63.88\pm0.42$ \\
\name                                   &     &            $\best{74.50}\pm0.23$ & & $\best{67.21}\pm0.25$ \\
\midrule
\midrule
CE                                   &     &            $78.6$ & & $64.2$ \\
Data Parameters            &     &            $78.5$ & & $64.5$ \\
DY-Bootstrap                   &     &           $74.2$ & & $61.6$ \\
INCV                                   &     &            $77.9$ & & $\best{66.7}$ \\
AUM                                   &     &            $\best{80.2}$ & & $66.5$ \\
\bottomrule
\end{tabular}
